Universal Adversarial Attacks with Natural Triggers for Text Classification

Recent work has demonstrated the vulnerability of modern text classifiers to universal adversarial attacks, which are input-agnostic sequences of words added to text processed by classifiers. Despite being successful, the word sequences produced in such attacks are often ungrammatical and can be easily distinguished from natural text. We develop adversarial attacks that appear closer to natural English phrases and yet confuse classification systems when added to benign inputs. We leverage an adversarially regularized autoencoder (ARAE) to generate triggers and propose a gradient-based search that aims to maximize the downstream classifier's prediction loss. Our attacks effectively reduce model accuracy on classification tasks while being less identifiable than prior models as per automatic detection metrics and human-subject studies. Our aim is to demonstrate that adversarial attacks can be made harder to detect than previously thought and to enable the development of appropriate defenses.

==> Tables/combined_table_dev-set_.tex <==
\begin{table*}[htb]
\centering
\renewcommand\arraystretch{1}
%\fontsize{10.5pt}{10.5pt}\selectfont
\resizebox{\textwidth}{!}{
\begin{tabular}{ccc|cc|cc}
\multicolumn{3}{c|}{} &  \multicolumn{2}{c|}{\large \textbf{NUTS (our model)}} & \multicolumn{2}{c}{\large \textbf{Baseline}~\cite{Wallace_uni_adv_NLP_EMNLP19}} \\
\multirow{2}{*}{\textbf{Task}} & \textbf{Trigger} & \textbf{Test} & \multirow{2}{*}{\textbf{Trigger}} & \textbf{Classifier} & \multirow{2}{*}{\textbf{Trigger}} & \textbf{Classifier}\\
 & \textbf{length} & \textbf{data} & & \textbf{accuracy} & & \textbf{accuracy} \\
\toprule

\multirow{10}{*}{\textbf{SST}} & \multirow{2}{*}{No trigger}  &  {\Large +} & - & 88.29\%  & - & 88.29\% \\

 & & {\Large -}  &  - & 82.94\% & - & 82.94\%\\ 
\cdashline{2-7}

%& \multirow{2}{*}{3}  &  {\Large +} & \emph{why none of} & 45.27\%  & \emph{drown soggy timeout} & 20.27\% \\
& \multirow{2}{*}{3}  &  {\Large +} & \emph{but neither the} & 40.54\%  & \emph{drown soggy timeout} & 20.27\% \\

%  & & {\Large -}  &   \emph{natural energy efficiency} & 23.60\% & \emph{vividly riveting soar} & 10.51\%\\ 
% \cdashline{2-7}
 & & {\Large -}  &   \emph{combined energy efficiency} & 21.26\% & \emph{vividly riveting soar} & 10.51\%\\ 
\cdashline{2-7}


 & \multirow{2}{*}{5}  &  {\Large +}   & \emph{a flat explosion empty over} & 26.35\% & \emph{drown soggy mixes soggy timeout} & 12.38\% \\
% \cmidrule{2-5}
& & {\Large -}  & \emph{they can deeply restore our} & 18.46\% & \emph{captures stamina lifetime without prevents} & 6.30\% \\
\cdashline{2-7}

 & \multirow{4}{*}{8} & \multirow{2}{*}{{\Large +}}   & \multirow{2}{4.8cm}{\emph{the accident forced the empty windows shut down}} & \multirow{2}{*}{27.25\%}  & \multirow{2}{6.2cm}{\emph{collapses soggy timeout energy energy freshness intellect genitals }} & \multirow{2}{*}{17.79\%}\\
& & &  & & & \\
% \cmidrule{2-5}
 & & \multirow{2}{*}{{\Large -}}  & \multirow{2}{4.8cm}{\emph{will deliver a deeply affected children from parents}} & \multirow{2}{*}{10.05\%} & \multirow{2}{6.2cm}{\emph{sunny vitality blessed lifetime lifetime counterparts without pitfalls}} & \multirow{2}{*}{1.87\%}\\
& & &  & & & \\
\midrule

\multirow{15}{*}{\textbf{SNLI}} & \multirow{3}{*}{No trigger}  &  {\Large +} & - & 90.95\%  & - & 90.95\% \\
& & 0 & - & 88.06\% & - & 88.06\% \\
 & & {\Large -}  &  - & 79.53\% & - & 79.53\%\\ 
\cdashline{2-7}

%  & \multirow{3}{*}{3} &  \Large + & \emph{she might not} & 1.02\% & \emph{alien spacecraft naked} & 0.00\%\\
 & \multirow{3}{*}{3} &  \Large + & \emph{he was jailed} & 0.03\% & \emph{alien spacecraft naked} & 0.00\%\\
& & 0 & \emph{there is no} & 2.53\% & \emph{spaceship cats zombies} & 0.00\% \\
& & \Large - & \emph{he could leave} & 54.58\%  & \emph{humans possesses energies} & 46.55\%\\
\cdashline{2-7}

% & \multirow{3}{*}{5}  &  \Large + & \emph{the new state won the} & 0.00\% & {\emph{alien spacecraft nothing eat no}} & {0.00\%}\\
 & \multirow{3}{*}{5}  &  \Large + & \emph{a man stabbed his son} & 0.00\% & {\emph{alien spacecraft nothing eat no}} & {0.00\%}\\
& & 0 & \emph{there is no one or} & 1.82\% & \emph{cats running indoors destroy no} & 0.00\%\\
% & & \Large - & \emph{he is hoping to assess} & 39.93\% & \emph{mammals tall beings interact near} & 13.24\%\\
& & \Large - & \emph{he likes to inspire creativity} & 39.48\% & \emph{mammals tall beings interact near} & 13.24\%\\
\cdashline{2-7}

% & \multirow{6}{*}{8} &  \multirow{2}{*}{\Large +} & \multirow{2}{4.8cm}{\emph{i read the crowd about the police after}} & \multirow{2}{*}{0.00\%}  & \multirow{2}{6.2cm}{\emph{mall destruction alien whatsoever shark pasture picnic no}} & \multirow{2}{*}{0.00\%}\\
& \multirow{6}{*}{8} &  \multirow{2}{*}{\Large +} & \multirow{2}{4.8cm}{\emph{some black women taking the photo last month}} & \multirow{2}{*}{0.00\%}  & \multirow{2}{6.2cm}{\emph{mall destruction alien whatsoever shark pasture picnic no}} & \multirow{2}{*}{0.00\%}\\
& & &  & & & \\
& & \multirow{2}{*}{0} & \multirow{2}{4.8cm}{\emph{the man drowned in hospital and died in}} & \multirow{2}{*}{3.74\%} & \multirow{2}{6.2cm}{\emph{cats rounds murder pandas in alien spacecraft mars}} & \multirow{2}{*}{0.00\%}\\
& & &  & & & \\
% & & \multirow{2}{*}{\Large -} & \multirow{2}{4.8cm}{\emph{he is seen after training trips to help}} & \multirow{2}{*}{26.08\%} & \multirow{2}{6.2cm}{\emph{human humans initiate accomplishment energies near objects near}} & \multirow{2}{*}{22.76\%}\\
& & \multirow{2}{*}{\Large -} & \multirow{2}{4.8cm}{\emph{they are helping for training achievement for a}} & \multirow{2}{*}{25.90\%} & \multirow{2}{6.2cm}{\emph{human humans initiate accomplishment energies near objects near}} & \multirow{2}{*}{22.76\%}\\
& & &  & & & \\

% \bottomrule
\end{tabular}
}
\caption{Universal attack results on both the Stanford Sentiment Treebank (SST) classifier and the Stanford Natural Language Inference (SNLI) classifier. For SST, ``+'' and ``-'' represent test sentences with positive sentiment and negative sentiment, respectively.
For SNLI, ``+'' , ``0'', and ``-'' represent test sentence pairs with entailment, neutral, and contradiction relations, respectively. 
We report the model accuracy after adding the attack triggers to benign test data (a lower accuracy means a more successful attack). `No trigger' refers to classifier accuracy without any attack.
Compared to the baseline~\cite{Wallace_uni_adv_NLP_EMNLP19}, our attack triggers are slightly less successful at reducing classifier accuracy but generate more natural triggers.
}
\label{tab:attack_results}
\end{table*}
